An elongated quantum dot as a distributed charge sensor

Increasing the separation between semiconductor quantum dots offers scaling advantages by fa- cilitating gate routing and the integration of sensors and charge reservoirs. Elongated quantum dots have been utilized for this purpose in GaAs heterostructures to extend the range of spin-spin interactions. Here, we study a metal-oxide-semiconductor (MOS) device where two quantum dot arrays are separated by an elongated quantum dot (340 nm long, 50 nm wide). We monitor charge transitions of the elongated quantum dot by measuring radiofrequency single-electron currents to a reservoir to which we connect a lumped-element resonator. We operate the dot as a single electron box to achieve charge sensing of remote quantum dots in each array, separated by a distance of 510 nm. Simultaneous charge detection on both ends of the elongated dot demonstrates that the charge is well distributed across its nominal length, supported by the simulated quantum-mechanical electron density. Our results illustrate how single-electron boxes can be realised with versatile foot- prints that may enable novel and compact quantum processor layouts, offering distributed charge sensing in addition to the possibility of mediated coupling.

==> IMEC-Metaltail Elongated single-electron box Arxiv/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR XELATEX
        system( "latexmk -cd -xelatex \"$_[0]\"" );
    }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR XELATEX
        system( "latexmk -cd -xelatex \"$_[0]\"" );
    }
}
